Learning Unbiased Representations via Mutual Information Backpropagation

We are interested in learning data-driven representations that can generalize well, even when trained on inherently biased data. In particular, we face the case where some attributes (bias) of the data, if learned by the model, can severely compromise its generalization properties. We tackle this problem through the lens of information theory, leveraging recent findings for a differentiable estimation of mutual information. We propose a novel end-to-end optimization strategy, which simultaneously estimates and minimizes the mutual information between the learned representation and the data attributes. When applied on standard benchmarks, our model shows comparable or superior classification performance with respect to state-of-the-art approaches. Moreover, our method is general enough to be applicable to the problem of ``algorithmic fairness'', with competitive results.

==> tab_cats_dogs.tex <==

\renewcommand{\arraystretch}{1.3}
\begin{wraptable}{r}{5.5cm}
% \begin{table}[!t]
\scriptsize
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{rcccccccccccccc}

\multicolumn{3}{c}{\footnotesize{\textbf{Cats \& Dogs experiment}}} \\

\toprule


& \multicolumn{1}{c}{\textbf{Train on TB1}} & \multicolumn{1}{c}{\textbf{Train on TB2}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5}

\textbf{Method} & \textbf{TB2}  & \textbf{TB1}  \\

\midrule

% & \multicolumn{4}{c}{\textbf{Learn Gender, Unlearn Age}}  \\

% \cmidrule(r){2-5}

ERM ($\lambda=0.0$) & $0.749\pm0.020$ & $0.692\pm0.007$ \\


Alvi et al.~\cite{zisserman2018} & $0.852$~\cite{kim2019cvpr}& $0.781$~\cite{kim2019cvpr} \\


Kim et al.~\cite{kim2019cvpr} & $0.903 $ & $0.873 $ \\


\textit{Ours} & $0.882$ & $0.793$ \\


\bottomrule
\end{tabular}}
\end{center}
\caption{\footnotesize ciao ciao.}

\label{tab:tab_cats_dogs}
\end{wraptable}
% \end{table}






==> tab_fairness_german.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table}[!t]
\scriptsize
\begin{center}
\resizebox{0.7\textwidth}{!}{
\begin{tabular}{rcccccccccccccc}

\multicolumn{6}{c}{\footnotesize{\textbf{German experiment}}} \\

\toprule

& \multicolumn{5}{c}{\textbf{Method}} \\
\cmidrule(r){2-6}

& SVM~\cite{donini2018empirical} & FERM~\cite{donini2018empirical} & NN~\cite{mary2019fairness} & NN + $\chi^2$~\cite{mary2019fairness} & \textit{Ours ($\lambda=1.0$)}\\

\midrule

Acc. & $0.74 \pm 0.03$ & $0.73 \pm 0.04$ & $0.74 \pm 0.04$ & $0.73 \pm 0.03$ & $0.72\pm 0.03$ \\


EO & $0.10 \pm 0.06 $ & $0.05 \pm 0.03$ & $0.47 \pm 0.19$ & $0.25 \pm 0.14$ & $0.05\pm 0.05$ \\


\bottomrule
\end{tabular}}
\end{center}
\caption{\footnotesize We compare against results as reported in~\cite{mary2019fairness}. For accuracy (first row), the higher the better. For EO (last row), the lower the better (\textit{i.e.}, the ``fairer''). Our results were averaged across $10$ different runs.}
\label{tab:german_results}
\end{table}


% \JC{Ci sono metodi di fairness su due parrocchie: alcuni ottimizzano per una metrica di fairness e testano sulla stessa [Donini ea], altri fanno cross metric [Mary ea], Noi siamo come i secondi more challenging.}

% \JC{Alcuni paper dicono che differenti nozioni di fairness incompatibili, noi famo vedere che EO e MI sono compatibili}



==> tab_imdb.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table}[t!]
\scriptsize
\begin{center}

\begin{tabular}{rcccc}

\multicolumn{5}{c}{} \\

\toprule


& \multicolumn{2}{c}{\textbf{Train on EB1}} & \multicolumn{2}{c}{\textbf{Train on EB2}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5}

\textbf{Method} & \textbf{EB2} & \textbf{Test} & \textbf{EB1} & \textbf{Test} \\

\midrule

ERM ($\lambda=0.0$) & $0.650\pm0.020$ & $0.849\pm0.007 $ & $0.576\pm0.013$ & $0.708\pm0.008$ \\
%ERM & $0.6503 \pm 0.020$ & $0.8493 \pm 0.007 $ & $0.5758 \pm .013$ & $0.7079 \pm 0.008$ \\

Alvi et al.~\cite{zisserman2018} & $0.637$~\cite{kim2019cvpr}& $0.856$~\cite{kim2019cvpr} & $0.573$~\cite{kim2019cvpr} & $0.699$~\cite{kim2019cvpr} \\
%Alvi et al.~\cite{zisserman2018} & $0.6374  $& $0.8556 $ & $0.5733 $ & $0.6990 $ \\

Kim et al.~\cite{kim2019cvpr} & $0.680 $ & $0.867 $ & $0.642$ & $0.745$ \\
%Kim et al.~\cite{kim2019cvpr} & $0.6800 $ & $0.8666 $ & $0.6418 $ & $0.7450 $ \\

\textit{Ours} & $0.684 \pm 0.010$ & $0.872 \pm 0.010$ & $0.631 \pm 0.034$ & $0.745 \pm 0.021$ \\
%\textit{Ours} & $0.6835 \pm 0.010 $ & $0.8718 \pm 0.010$ & $0.5955\pm 0.005$ & $0.7226 \pm 0.003$ \\

\bottomrule
\end{tabular}
\end{center}
\caption{\footnotesize \textbf{IMDB experiment -- comparison with related work.} The first row reports results obtained by setting $\lambda=0.0$ (ERM baseline). The last row reports results obtained with our method (\textit{Ours}), by setting $\lambda=0.5$ for EB1 and $\lambda=0.9$ for EB2. Each column reports results associated with the indicated test set.}
% \caption{\footnotesize Train on EB1: lmb 0.5 iterMI 40 iteracc 10 lrM 0.1. Train on EB2: lmb_0.8_iter_MI_60_iter_acc_10_lr_M_0.1 \ric{reminder: discorso baseline diverse} \ric{tolto learn Age}}
\label{tab:tab_imdb}
\end{table}

==> table_merged.tex <==
\begin{table}
    \parbox{.45\linewidth}{
        \centering
        \scalebox{.6}{% IMDB TABLE --------------------------
        \begin{tabular}{rcccccccccccccc}

            \multicolumn{5}{c}{\footnotesize{\textbf{IMBD experiment}}} \\
            
            \toprule
            
            
            & \multicolumn{2}{c}{\textbf{Train on EB1}} & \multicolumn{2}{c}{\textbf{Train on EB2}} \\
            
            \cmidrule(r){2-3} \cmidrule(r){4-5}
            
            \textbf{Method} & \textbf{EB2} & \textbf{Test} & \textbf{EB1} & \textbf{Test} \\
            
            \midrule
            
            % & \multicolumn{4}{c}{\textbf{Learn Gender, Unlearn Age}}  \\
            
            % \cmidrule(r){2-5}
            
            ERM ($\lambda=0.0$) & $0.650\pm0.020$ & $0.849\pm0.007 $ & $0.576\pm0.013$ & $0.708\pm0.008$ \\
            %ERM & $0.6503 \pm 0.020$ & $0.8493 \pm 0.007 $ & $0.5758 \pm .013$ & $0.7079 \pm 0.008$ \\
            
            Alvi et al.~\cite{zisserman2018} & $0.637$~\cite{kim2019cvpr}& $0.856$~\cite{kim2019cvpr} & $0.573$~\cite{kim2019cvpr} & $0.699$~\cite{kim2019cvpr} \\
            %Alvi et al.~\cite{zisserman2018} & $0.6374  $& $0.8556 $ & $0.5733 $ & $0.6990 $ \\
            
            Kim et al.~\cite{kim2019cvpr} & $0.680 $ & $0.867 $ & $0.642$ & $0.745$ \\
            %Kim et al.~\cite{kim2019cvpr} & $0.6800 $ & $0.8666 $ & $0.6418 $ & $0.7450 $ \\
            
            \textit{Ours} & $0.684 \pm 0.010$ & $0.872 \pm 0.010$ & $0.6279 \pm 0.036$ & $0.744 \pm 0.022$ \\
            
            
            \bottomrule
            \end{tabular}
        }
        \caption{IMDB CAPTION}
        \label{tab:imdb}
    }
    \hfill
    \parbox{.45\linewidth}{
        \centering
        \scalebox{.6}{% dogs---------------
            \begin{tabular}{rcccccccccccccc}

\multicolumn{3}{c}{\footnotesize{\textbf{Cats \& Dogs experiment}}} \\

\toprule


& \multicolumn{1}{c}{\textbf{Train on TB1}} & \multicolumn{1}{c}{\textbf{Train on TB2}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5}

\textbf{Method} & \textbf{TB2}  & \textbf{TB1}  \\

\midrule

% & \multicolumn{4}{c}{\textbf{Learn Gender, Unlearn Age}}  \\

% \cmidrule(r){2-5}

ERM ($\lambda=0.0$) & $0.749\pm0.020$ & $0.692\pm0.007$ \\


Alvi et al.~\cite{zisserman2018} & $0.852$~\cite{kim2019cvpr}& $0.781$~\cite{kim2019cvpr} \\


Kim et al.~\cite{kim2019cvpr} & $0.903 $ & $0.873 $ \\


\textit{Ours} & $0.882$ & $0.793$ \\


\bottomrule
\end{tabular}
        }
        \caption{Cats caption}
        \label{tab:cats_dogs}
    }
\end{table}
